On the Impact and Utility of Single-Exomoon Modeling for Multi-Moon Systems

The search for exomoons in time-domain photometric data has to-date generally consisted of fitting transit models that are comprised of a planet hosting a single moon. This simple model has its advantages, but it may not be particularly representative, as most of the major moons in our Solar System are found in multi-moon satellite systems. It is critical that we investigate, then, the impact of applying a single-moon model to systems containing multiple moons, as there is the possibility that utilizing an inaccurate or incomplete model could lead to erroneous conclusions about the system. To that end, in this work we produce a variety of realistic multi-moon light curves, perform standard single-moon model selection, and analyze the impacts that this model choice may have on the search for exomoons. We find that the number of moons in a system fit with a single-moon model generally has little impact on whether we find evidence for a moon in that system, and other system attributes are individually not especially predictive. However, the model parameter solutions for the moon frequently do not match any real moon in the system, instead painting a picture of a ``phantom'' moon. We find no evidence that multi-moon systems yield corresponding multi-modal posteriors. We also find a systematic tendency to overestimate planetary impact parameter and eccentricity, to derive unphysical moon densities, and to infer potentially unphysical limb darkening coefficients. These results will be important to keep in mind in future exomoon search programs.

==> sim_table.tex <==
\begin{table*}
    \renewcommand{\arraystretch}{1.3}
  \centering
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
    \textbf{Number of moons} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} \\
    \hline 
    \hline
    Total (fixed host) & 14819 & 5157 & 11612 & 10028 & 8384 \\
    \hline
    Total (\%) stable & 14793 (99.8\%) & 4752 (92.1\%) & 2694 (23.2\%) & 739 (7.4\%) & 161 (1.9\%) \\
    %\hline
    + $\Delta\mathrm{BIC} \leq -2$ & 12300 (83.0\%) & 3834 (74.3\%) & 1986 (17.1\%) & 448 (4.5\%) & 76 (0.9\%) \\
    %\hline
    + cross-validated & 11835 (79.9\%) & 3668 (71.1\%) & 1862 (16.0\%) & 414 (4.1\%) & 70 (0.8\%) \\
    \hline
    %Total (\%) remaining & --- & --- & --- & --- & --- \\
    %\hline
    + $\Delta\mathrm{AIC} \leq 0$ & 14033 (94.7\%) & 4527 (87.8\%) & 2460 (21.2\%) & 621 (6.2\%) & 121 (1.4\%) \\
    %\hline
    + cross-validated & 13433 (90.6\%) & 4311 (83.6\%) & 2311 (19.9\%) & 574 (5.7\%) & 112 (1.3\%) \\
    \hline
    $P_{\mathrm{TTV}}$ [epochs] & $3.41^{+4.73}_{-1.19}$ & $3.38\,^{+3.94}_{-1.15}$ & $3.25\,^{+3.52}_{-1.11}$ & $3.49\,^{+2.56}_{-1.48}$ & $3.04\,^{+3.71}_{-0.99}$ \\[3pt]
    \hline
    $A_{\mathrm{TTV}}$ [min] & $1.84^{+11.38}_{-1.37}$ & $1.37\,^{+6.85}_{-0.97}$ & $1.46\,^{+10.22}_{-1.0}$ & $1.47\,^{+15.27}_{-0.99}$ & $0.70\,^{+5.34}_{-0.36}$ \\[3pt]
    \hline
    $(\sum M_S) \, / \, M_P$ & $5.5^{+3.1}_{-3.3} \times 10^{-3}$ & $5.5\,^{+3.2}_{3.3} \times 10^{-3}$ & $3.9\,^{+3.7}_{-2.6} \times 10^{-3}$ & $2.7\,^{+3.6}_{-2.1} \times 10^{-3}$ & $6.7\,^{+31.9}_{-5.5} \times 10^{-4}$ \\[3pt]
    \hline
    \hline
    Total (variable host) & 15421 & 5148 & 11596 & 9486 & 7773 \\
    \hline
    Total (\%) stable & 15392 (99.8\%) & 4732 (91.9\%) & 2549 (22.0\%) & 550 (5.8\%) & 149 (1.9\%) \\
    %\hline
    + $\Delta\mathrm{BIC} \leq -2$ & 6418 (41.6\%) & 1905 (37.0\%) & 880 (7.6\%) & 173 (1.8\%) & 34 (0.4\%) \\
    %\hline
    + cross-validated & 6217 (39.9\%) & 1856 (35.6\%) & 827 (7.0\%) & 158 (1.6\%) & 34 (0.4\%) \\
    \hline
    + $\Delta\mathrm{AIC} \leq 0$ & 12489 (80.1\%) & 3812 (73.1\%) & 1788 (15.2\%) & 333 (3.5\%) & 87 (1.1\%) \\
    %\hline
    + cross-validated & 11803 (75.7\%) & 3619 (69.4\%) & 1666 (14.2\%) & 299 (3.1\%) & 83 (1.1\%) \\
    \hline    
    $P_{\mathrm{TTV}}$ [epochs] & $3.44\,^{+4.21}_{-1.15}$ & $3.42\,^{+4.06}_{-1.17}$ & $3.24\,^{+3.13}_{-0.98}$ & $3.3\,^{+2.16}_{-0.89}$ & $3.73\,^{+3.61}_{-1.36}$ \\[3pt]
    \hline
    $A_{\mathrm{TTV}}$ [min] & $2.96\,^{+5.87}_{-2.02}$ & $2.65\,^{+5.14}_{-1.79}$ & $2.8\,^{+5.06}_{-1.87}$ & $2.6\,^{+5.34}_{-1.71}$ & $2.37\,^{+7.69}_{-1.86}$ \\[3pt]
    \hline
    $(\sum M_S) \, / \, M_P$ & $5.6\,^{+3.1}_{-3.5} \times 10^{-3}$ & $5.5\,^{+3.2}_{-3.5} \times 10^{-3}$ & $3.3\,^{+4.2}_{-2.6} \times 10^{-3}$ & $1.5\,^{+4.6}_{-1.2} \times 10^{-3}$ & $4.4\,^{+9.7}_{-3.7} \times 10^{-4}$ \\[3pt]
    \hline
    \hline
    Total (resonant chain) & 15012 & 4839 & 12522 & 10251 & 7376 \\
    \hline
    Total (\%) stable & 14983 (99.8\%) & 4381 (90.5\%) & 1429 (11.4\%) & 455 (4.4\%) & 168 (2.3\%) \\
    %\hline
    + $\Delta\mathrm{BIC} \leq -2$ & 6125 (40.8\%) & 1529 (31.6\%) & 460 (3.7\%) & 127 (1.2\%) & 41 (0.6\%)  \\
    %\hline
    + cross-validated & 5833 (38.9\%) & 1471 (30.4\%) & 446 (3.6\%) & 125 (1.2\%) & 39 (0.5\%) \\
    \hline
    + $\Delta\mathrm{AIC} \leq 0$ & 12130 (80.8\%) & 3434 (71.0\%) & 1059 (8.5\%) & 301 (2.9\%) & 100 (1.4\%) \\
    %\hline
    + cross-validated & 11475 (76.4\%) & 3256 (67.3\%) & 1006 (8.0\%) & 284 (2.8\%) & 94 (1.3\%) \\
    \hline    
    $P_{\mathrm{TTV}}$ [epochs] & $3.42\,^{+3.98}_{-1.15}$ & $3.45\,^{+4.65}_{-1.17}$ & $3.49\,^{+3.61}_{-1.21}$ & $3.43\,^{+3.71}_{-1.23}$ & $4.05\,^{+2.26}_{-1.41}$ \\[3pt]
    \hline
    $A_{\mathrm{TTV}}$ [min] & $2.91\,^{+6.1}_{-1.99}$ & $2.38\,^{+4.78}_{-1.63}$ & $2.11\,^{+4.1}_{-1.45}$ & $2.32\,^{+4.61}_{-1.62}$ & $2.01\,^{+5.17}_{-1.51}$ \\[3pt]
    \hline
    $(\sum M_S) \, / \, M_P$ & $5.5\,^{+3.2}_{-3.4} \times 10^{-3}$ & $5.5\,^{+3.0}_{-3.7} \times 10^{-3}$ & $2.6\,^{+2.7}_{-2.1} \times 10^{-3}$ & $1.5\,^{+3.4}_{-1.3} \times 10^{-3}$ & $7.0\,^{+27.9}_{-5.2} \times 10^{-4}$ \\[3pt]
    \hline
    
 \end{tabular}
  \caption{Summary of the ``fixed host'' (top five rows) and ``variable host'' (middle five rows) and ``resonant chain'' (bottom five rows) simulations produced for this work. Percentages quoted indicate the fraction of total generated systems. Values quoted for $P_{\mathrm{TTV}}$, $A_{\mathrm{TTV}}$, and total satellite mass ratios are the median and 1$\sigma$ values for the robust cross-validation sample using $\Delta$BIC as the selection metric.}
  \label{tab:summary}
\end{table*}
